Modulo-$(2^{2n}+1)$ Arithmetic via Two Parallel n-bit Residue Channels

Augmenting the balanced residue number system moduli-set $\{m_1=2^n,m_2=2^n-1,m_3=2^n+1\}$, with the co-prime modulo $m_4=2^{2n}+1$, increases the dynamic range (DR) by around 70%. The Mersenne form of product $m_2 m_3 m_4=2^{4n}-1$, in the moduli-set $\{m_1,m_2,m_3,m_4\}$, leads to a very efficient reverse convertor, based on the New Chinese remainder theorem. However, the double bit-width of the m_4 residue channel is counter-productive and jeopardizes the speed balance in $\{m_1,m_2,m_3\}$. Therefore, we decompose $m_4$ to two complex-number n-bit moduli $2^n\pm\sqrt{-1}$, which preserves the DR and the co-primality across the augmented moduli set. The required forward modulo-$(2^{2n}+1)$ to moduli-$(2^n\pm\sqrt{-1}) $conversion, and the reverse are immediate and cost-free. The proposed unified moduli-$(2^n\pm\sqrt{-1})$ adder and multiplier, are tested and synthesized using Spartan 7S100 FPGA. The 6-bit look-up tables (LUT), therein, promote the LUT realizations of adders and multipliers, for $n=5$, where the DR equals $2^{25}-2^5$. However, the undertaken experiments show that to cover all the 32-bit numbers, the power-of-two channel $m_1$ can be as wide as 12 bits with no harm to the speed balance across the five moduli. The results also show that the moduli-$(2^5\pm\sqrt{-1})$ add and multiply operations are advantageous vs. moduli-$(2^5\pm1)$ in speed, cost, and energy measures and collectively better than those of modulo-$(2^{10}+1)$.

==> Sections/ConcludingRemarks.tex <==
\section{Concluding Remarks}
In conclusion, this paper has introduced a novel representation that replaces the traditional modulo-$(2^{2n}+1)$ with moduli-$(2^n\pm \sqrt{-1})$, which results in a more balanced and efficient moduli set. 
The proposed moduli set offers a promising alternative to conventional approaches, particularly in the context of RNS-CNN and RNS-DNN applications. 
The synthesis results have demonstrated the potential benefits of adopting this novel moduli set, suggesting that it could pave the way for improved performance and resource utilization in various RNS arithmetic applications. 
This innovation holds the potential to enhance the efficiency and effectiveness of hardware implementations for a wide range of computational tasks, offering a valuable contribution to the field of digital design and signal processing. 
Also, we have leveraged the Xilinx Spartan 7S100 FPGA platform as our design framework. The Spartan 7 FPGA series featuring 6-bit LUTs offers optimal resource utilization and performance.
